EMPHATIC: A proposed experiment to measure hadron scattering and productioncross sections for improved neutrino flux predictions

Hadron scattering and production uncertainties are a limiting systematic on accelerator and at-mospheric neutrino flux predictions. New hadron measurements are necessary for neutrino fluxpredictions with well-understood and reduced uncertainties. We propose a new compact experimentto measure hadron scattering and production cross sections at beam energies that are inaccessibleto currently operating experiments. These measurements can reduce the current 10% neutrino fluxuncertainties by an approximate factor of two.

==> EMPHATIC Proposal/authors.tex <==
\newcommand{\FNAL}{Fermi National Accelerator Laboratory, Batavia, 
Illinois 60510, USA}
\newcommand{\TRIUMF}{TRIUMF, Vancouver, BC  V6T 2A3, Canada}
\newcommand{\KEK}{Institute of
Particle and Nuclear Study (IPNS), High Energy Accelerator Research
Organization (KEK), Tsukuba, 305-0801, Japan}
\newcommand{\IPMU}{IPMU, Kashiwa, Chiba 277-8583, Japan}
\newcommand{\Nagoya}{Nagoya University, Nagoya, Aichi 464-8601, Japan}
\newcommand{\Kyoto}{Kyoto University, Yoshidahonmachi, Kyoto, Kyoto 606-8501, Japan}
\newcommand{\Winnipeg}{University of Winnipeg, Winnipeg, MB R3B 2E9, Canada}
\newcommand{\Chiba}{Department of Physics, Chiba University, Chiba, Chiba 263-8522, Japan}
\newcommand{\RCNP}{Research Center for Nuclear Physics (RCNP), Ibaraki,
567-0047, Japan}
\newcommand{\Osaka}{Department of Physics, Osaka University, Toyonaka 560-0043, Japan}
\newcommand{\RIKEN}{RIKEN, Wako, 351-0198, Japan}
\newcommand{\Sinica}{Institute of Physics, Academia Sinica, Taipei 11529, Taiwan}
\newcommand{\Tohoku}{Department of Physics, Tohoku University, Sendai 980-8578, Japan}
\newcommand{\ELPH}{Research Center for Electron Photon Science (ELPH), Tohoku University, Sendai, 982-0826, Japan}
\newcommand{\OsakaCity}{Department of Physics, Osaka City University, Osaka 558-8585, Japan}
\newcommand{\Kobe}{Kobe University, Kobe, Hyogo 657-8501, Japan}
\newcommand{\Regina}{Department of Physics, University of Regina, SK, S4S 0A2, Canada}
\newcommand{\York}{York University, Department of Physics and Astronomy, Toronto, Ontario, Canada}
\newcommand{\Wichita}{Department of Mathematics, Statistics, and Physics, Wichita State University, Wichita, Kansas 67206, USA}
\newcommand{\Boston}{Department of Physics, Boston University, Boston, Massachusetts, USA}
\newcommand{\WilliamMary}{Department of Physics, College of William \& Mary, Williamsburg, Virginia 23187, USA}
\newcommand{\Cincinnati}{Department of Physics, University of Cincinnati, Cincinnati, Ohio 45221, USA}
\newcommand{\SDSMT}{South Dakota School of Mines and Technology, Rapid City, South Dakota 57701, USA}
\newcommand{\UTA}{Department of Physics, University of Texas at Austin, Austin, TX 78712, USA}


\affiliation{\Boston}
\affiliation{\Chiba}
\affiliation{\Cincinnati}
\affiliation{\FNAL}
\affiliation{\KEK}
\affiliation{\Sinica}
\affiliation{\IPMU}
\affiliation{\Kobe}
\affiliation{\Kyoto}
\affiliation{\Nagoya}
\affiliation{\OsakaCity}
\affiliation{\Osaka}
\affiliation{\RCNP}
\affiliation{\Regina}
\affiliation{\Tohoku}
\affiliation{\ELPH}
\affiliation{\RIKEN}
\affiliation{\SDSMT}
\affiliation{\UTA}
\affiliation{\TRIUMF}
\affiliation{\Wichita}
\affiliation{\WilliamMary}
\affiliation{\Winnipeg}
\affiliation{\York}

\author{T.~Akaishi}
\affiliation{\Osaka}

\author{L.~Aliaga-Soplin}
\affiliation{\FNAL}

\author{H.~Asano}
\affiliation{\RIKEN}

\author{A.~Aurisano}
\affiliation{\Cincinnati}

\author{M.~Barbi}
\affiliation{\Regina}

\author{L.~Bellantoni}
\affiliation{\FNAL}

\author{S.~Bhadra}
\affiliation{\York}

\author{W-C.~Chang} 
\affiliation{\York}

\author{L.~Fields}
\affiliation{\FNAL}

\author{A.~Fiorentini} 
\affiliation{\SDSMT}

\author{M.~Friend}
\affiliation{\KEK}

\author{T.~Fukuda}
\affiliation{\Nagoya}

\author{D.~Harris}
\affiliation{\FNAL}

\author{M.~Hartz}
\affiliation{\IPMU}
\affiliation{\TRIUMF}

\author{R.~Honda} 
\affiliation{\Tohoku}

\author{T.~Ishikawa} 
\affiliation{\ELPH}

\author{B.~Jamieson}
\affiliation{\Winnipeg}

\author{E.~Kearns}
\affiliation{\Boston}

\author{N.~Kolev}
\affiliation{\Regina}

\author{M.~Komatsu} 
\affiliation{\Nagoya}

\author{Y.~Komatsu} 
\affiliation{\KEK}

\author{A.~Konaka}
\affiliation{\TRIUMF}

\author{M.~Kordosky}
\affiliation{\WilliamMary}

\author{K.~Lang}
\affiliation{\UTA}

\author{P.~Lebrun}
\affiliation{\FNAL}

\author{T.~Lindner}
\affiliation{\Winnipeg}
\affiliation{\TRIUMF}

\author{Y.~Ma}
\affiliation{\RIKEN}

\author{D.~A.~Martinez Caicedo}
\affiliation{\SDSMT}

\author{M.~Muether}
\affiliation{\Wichita}

\author{N.~Naganawa} 
\affiliation{\Nagoya}

\author{M.~Naruki} 
\affiliation{\Kyoto}

\author{E.~Niner} 
\affiliation{\FNAL}

\author{H.~Noumi}
\affiliation{\RCNP}

\author{K.~Ozawa} 
\affiliation{\KEK}

\author{J.~Paley}
\thanks{Co-spokesperson: Jonathan M. Paley (jpaley@fnal.gov)}
\affiliation{\FNAL}

\author{M.~Pavin}
\affiliation{\TRIUMF}

\author{P.~de Perio}
\affiliation{\TRIUMF}

\author{M.~Proga}
\affiliation{\UTA}

\author{F.~Sakuma}
\affiliation{\RIKEN}

\author{G.~Santucci} 
\affiliation{\York}

\author{T.~Sawada} 
\affiliation{\OsakaCity}

\author{O.~Sato} 
\affiliation{\Nagoya}

\author{T.~Sekiguchi}
\thanks{Co-spokesperson: Tetsuro Sekiguchi (tetsuro.sekiguchi@kek.jp)}
\affiliation{\KEK}

\author{K.~Shirotori}
\affiliation{\RCNP}

\author{A.~Suzuki} 
\affiliation{\Kobe}

\author{M.~Tabata}
\affiliation{\Chiba}

\author{T.~Takahashi}
\affiliation{\RCNP}

\author{N.~Tomida}
\affiliation{\RCNP}

\author{R.~Wendell}
\affiliation{\Kyoto}

\author{T.~Yamaga}
\affiliation{\RIKEN}

\collaboration{The EMPHATIC Collaboration}
\noaffiliation

